Hypothesis testing for eigenspaces of covariance matrix

Eigenspaces of covariance matrices play an important role in statistical machine learning, arising in variety of modern algorithms. Quantitatively, it is convenient to describe the eigenspaces in terms of spectral projectors. This work focuses on hypothesis testing for the spectral projectors, both in one- and two-sample scenario. We present new tests, based on a specific matrix norm developed in order to utilize the structure of the spectral projectors. A new resampling technique of independent interest is introduced and analyzed: it serves as an alternative to the well-known multiplier bootstrap, significantly reducing computational complexity of bootstrap-based methods. We provide theoretical guarantees for the type-I error of our procedures, which remarkably improve the previously obtained results in the field. Moreover, we analyze power of our tests. Numerical experiments illustrate good performance of the proposed methods compared to previously developed ones.

==> source/BayesLink.tex <==
Let's apply Bayesian methods to resolve this problem. Let $\Pi$ be a prior distribution on the set of covariance matrices $ \Su $.
The Gaussian log-likelihood:
\begin{equation}
    \begin{aligned}
    \ell_{n}(\Su) 
    = 
    - \frac{n}{2}\log{\det(\Su)} 
    - \frac{n}{2} \Tr(\Su^{-1}\Se) 
    - \frac{nd}{2} \log{(2\pi)}.
    \nonumber
    \end{aligned}
\end{equation}
The posterior measure of a set $ \mathcal{A} \subset \SPD $ is expressed as
\begin{equation}
    \begin{aligned}
    \Pi(\mathcal{A}|\data) 
    = 
    \frac{\int_{\mathcal{A}} {\exp{\left(\ell_{n}(\Su) \right)} \;d\Pi(\Su)}}{\int_{\SPD}
    	 {\exp{\left(\ell_{n}(\Su)\right)} \;d\Pi(\Su)}}\,.
\nonumber
    \end{aligned}
\end{equation}
Once a prior is fixed, we can easily sample matrices $ \Su $ from this posterior distribution.

It turns out to be convenient to focus on the conjugate prior to the multivariate Gaussian distribution, that is, the Inverse Wishart distribution $ \mathcal{IW}_{d}(\G, d+b-1) $ with parameters $ \G \in \SPD$ , $ 0 < b \lesssim d $.
As this distribution is conjugate to the Gaussian, the posterior distribution belongs to the same family; in particular, $\Pi(\Su|\data)$ is $ \mathcal{IW}_{d}(\G+n\Se, n+d+b-1) $. We will actively use the following well-known property of the Inverse Wishart distribution:
\begin{equation}
    \begin{aligned}
	\Su^{-1} \;|\; \data 
	& \stackrel{d}{=} &
	\sum_{j=1}^{n+d+b-1} W_j W_j^{\T} \;|\; \data,  
\nonumber
    \end{aligned}
\end{equation}
where $ W_j \;|\; \data \stackrel{i.i.d.}{\sim} \mathcal{N}(0, (\G + n\Se)^{-1}) $. 
Introducing for shortness the notations
\begin{equation}
    \begin{aligned}
    n_d  := n+d+b-1 \;\text{ (with } b \lesssim d \text{) and }\;
	\Su_{n,d} 
	& := &
	\frac{1}{n_d} \G + \frac{n}{n_d} \Se,
\nonumber
    \end{aligned}
\end{equation}
we can rewrite
\begin{equation}
    \begin{aligned}
	\Su^{-1} \;|\; \data 
	& \stackrel{d}{=} &
	\Su_{n,d}^{-1/2}\left(\frac{1}{n_d}\sum_{j=1}^{n_d} Z_j Z_j^{\T} \right)\Su_{n,d}^{-1/2}\;|\; \data,  
\nonumber
    \end{aligned}
\end{equation}
where $ Z_j \;|\; \data \stackrel{i.i.d.}{\sim} \mathcal{N}(0, \Id_d) $.
After some technical computations it can be shown that
\begin{equation}
    \begin{aligned}
	(\Su - \Se) \;|\; \data 
	& \stackrel{d}{\approx} &
	-\Su_{n,d}^{1/2}\left(\frac{1}{n_d}\sum_{j=1}^{n_d} Z_j Z_j^{\T} - \Id_d \right)\Su_{n,d}^{1/2}\;|\; \data \stackrel{d}{=} -\left( \frac{1}{n_d}\sum_{j=1}^{n_d} V_j V_j^{\T} - \Su_{n,d} \right) \;\bigg|\; \data
\nonumber
    \end{aligned}
\end{equation}
with $V_j \;|\; \data \stackrel{i.i.d.}{\sim} \mathcal{N}(0, \Su_{n,d})$.

So, if we verify that with high probability
\begin{equation}
    \begin{aligned}
	\sqrt{n}\,\| \Su - \Se\|_{\infty} \;|\; \data 
	& \stackrel{d}{\approx} &
	\sqrt{n}\,\| \Se - \St\|_{\infty},
\nonumber
    \end{aligned}
\end{equation}
then we can use the quantiles of $\sqrt{n}\,\| \Su - \Se\|_{\infty} \;|\; \data$, which is completely under our control and can be simulated, instead of the true quantiles in order to build the sharp confidence sets of the described form for $\St$.

==> source/proofs/Proof_Power2.tex <==
Again, we prove only (i). We start the proof similarly to the previous one.
\begin{equation}
    \begin{aligned}
        &\Prob\left[ \sqrt{\frac{n_an_b}{n_a+n_b}} \| \Pea - \Peb\|_{(\Pbar, \overline{\Gamma}, s_1, s_2)} \geq \gamma_B^{(2)}(\alpha) \right]
        \geq \\
        &\qquad \geq 
        \Prob\left[ \sqrt{\frac{n_an_b}{n_a+n_b}} \| \Pta - \Ptb\|_{(\Pbar, \overline{\Gamma}, s_1, s_2)} - \sqrt{\frac{n_an_b}{n_a+n_b}} \| (\Pea-\Pta) - (\Peb-\Ptb)\|_{(\Pbar, \overline{\Gamma}, s_1, s_2)} \geq \gamma_B^{(2)}(\alpha) \right].
    \nonumber
    \end{aligned}
\end{equation}
Here, unlike the previous proof, we apply our equivalence of norms Proposition~\ref{P:Properties0} (ii), and the assumption of the theorem:
\begin{equation}
    \begin{aligned}
        \| \Pta - \Ptb\|_{(\Pbar, \overline{\Gamma}, s_1, s_2)}
        \geq \frac{1}{2}\cdot\frac{s_1}{m}\cdot\frac{s_2}{d-m}\cdot \| \Pta - \Ptb\| \geq \frac{\lambda_{n_a, n_b}}{\sqrt{n_an_b/(n_a+n_b)}}.
    \nonumber
    \end{aligned}
\end{equation}
Thus,
\begin{equation}
    \begin{aligned}
        &\Prob\left[ \sqrt{\frac{n_an_b}{n_a+n_b}} \| \Pea - \Peb\|_{(\Pbar, \overline{\Gamma}, s_1, s_2)} \geq \gamma_B^{(2)}(\alpha) \right]
        \geq \\
        &\qquad \geq 
        \Prob\left[ \lambda_{n_a,n_b} - \sqrt{\frac{n_an_b}{n_a+n_b}} \| (\Pea-\Pta) - (\Peb-\Ptb)\|_{(\Pbar, \overline{\Gamma}, s_1, s_2)} \geq \gamma_B^{(2)}(\alpha) \right].
    \nonumber
    \end{aligned}
\end{equation}
The rest of the proof repeats the previous one.
